Conditional Deformable Image Registration with Spatially-Variant and Adaptive Regularization

Deep learning-based image registration approaches have shown competitive performance and run-time advantages compared to conventional image registration methods. However, existing learning-based approaches mostly require to train separate models with respect to different regularization hyperparameters for manual hyperparameter searching and often do not allow spatially-variant regularization. In this work, we propose a learning-based registration approach based on a novel conditional spatially adaptive instance normalization (CSAIN) to address these challenges. The proposed method introduces a spatially-variant regularization and learns its effect of achieving spatially-adaptive regularization by conditioning the registration network on the hyperparameter matrix via CSAIN. This allows varying of spatially adaptive regularization at inference to obtain multiple plausible deformations with a single pre-trained model. Additionally, the proposed method enables automatic hyperparameter optimization to avoid manual hyperparameter searching. Experiments show that our proposed method outperforms the baseline approaches while achieving spatially-variant and adaptive regularization.

==> Figures/table.tex <==
\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{}     & Avg.Dice Score & Avg.$|J_{\phi}|<0$\% & Avg.$|\nabla J_{\phi}|$ & \multicolumn{1}{l|}{Std$|J_{\phi}|$} & Avg. Regularization Hyperparameter $\vec{\lambda}$ \\ \hline
CSAIN with $\Lambda_{gau}$ & 0.761          & 1.16                 & 0.00070                 & 0.0063                               & $[4.01, 1.96, 2.19, 2.10, 2.07]$                  \\ \hline
CSAIN with $\Lambda$       & 0.758          & 1.49                 & 0.00068                 & 0.0061                               & $[3.45, 1.31, 1.62, 1.91, 1.50]$                   \\ \hline
CIR-DM                     & 0.749          & 0.66                 & 0.00100                 & 0.0094                               & 1.0                                                \\ \hline
\end{tabular}
\caption{Quantitative results on OASIS dataset using CSAIN and CIR-DM. Average Dice Score of different anatomical structures across test set. $|J_{\phi}|<0\%$ is the percentage of points with a negative Jacobian Determinant, higher means more folding. $|\nabla J_{\phi}|$ is the gradient of the Jacobian Determinant, lower value means a smoother deformation field.}
\label{table:results}
\end{table*}

==> name.tex <==
\begin{table*}[]
\begin{tabular}{|l|lllll|lllll|}
\hline
              & \multicolumn{5}{c|}{Dice Score}                                                                                          & \multicolumn{5}{c|}{Jacobian Det}                                                                \\ \hline
              & \multicolumn{1}{l|}{$\lambda_{0}$} & \multicolumn{1}{l|}{$\lambda_{1}$} & \multicolumn{1}{l|}{$\lambda_{2}$} & \multicolumn{1}{l|}{$\lambda_{3}$} & $\lambda_{4}$ & \multicolumn{1}{l|}{$\lambda_{0}$} & \multicolumn{1}{l|}{$\lambda_{1}$} & \multicolumn{1}{l|}{$\lambda_{2}$} & \multicolumn{1}{l|}{$\lambda_{3}$} & $\lambda_{4}$ \\ \hline
$\lambda = 2$ & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \hline
$\lambda = 5$ & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \hline
$\lambda = 8$ & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{}             & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \hline
\end{tabular}
\end{table*}
